UniAct: Unified Motion Generation and Action Streaming for Humanoid Robots

A long-standing objective in humanoid robotics is the realization of versatile agents capable of following diverse multimodal instructions with human-level flexibility. Despite advances in humanoid control, bridging high-level multimodal perception with whole-body execution remains a significant bottleneck. Existing methods often struggle to translate heterogeneous instructions -- such as language, music, and trajectories -- into stable, real-time actions. Here we show that UniAct, a two-stage framework integrating a fine-tuned MLLM with a causal streaming pipeline, enables humanoid robots to execute multimodal instructions with sub-500 ms latency. By unifying inputs through a shared discrete codebook via FSQ, UniAct ensures cross-modal alignment while constraining motions to a physically grounded manifold. This approach yields a 19% improvement in the success rate of zero-shot tracking of imperfect reference motions. We validate UniAct on UniMoCap, our 20-hour humanoid motion benchmark, demonstrating robust generalization across diverse real-world scenarios. Our results mark a critical step toward responsive, general-purpose humanoid assistants capable of seamless interaction through unified perception and control.

==> supp_v1_submission.tex <==
\clearpage
\appendix
\renewcommand\thefigure{A\arabic{figure}}
\setcounter{figure}{0}
\renewcommand\thetable{A\arabic{table}}
\setcounter{table}{0}
\renewcommand\theequation{A\arabic{equation}}
\setcounter{equation}{0}
\pagenumbering{arabic}% resets `page` counter to 1
\renewcommand*{\thepage}{A\arabic{page}}
\setcounter{footnote}{0}

% \begin{@twocolumnfalse}
%     \centering
%     \Large\bfseries Supplementary Material for\\[2ex]
%     % \normalsize Author Name\\[1ex]
%     % \today
%     \vspace{2ex}
% \end{@twocolumnfalse}


\maketitlesupplementary


\section{Additional qualitative results}

We present extensive qualitative results of real-world experiments across different modalities: language-to-motion (\cref{fig:text2motion_qual}), music-to-motion (\cref{fig:music2motion_qual}), trajectory-to-motion (\cref{fig:traj2motion_qual}), and human-to-humanoid motion (\cref{fig:gvmhr2motion_qual}). These results demonstrate that UniAct possesses diverse instruction following capabilities and exhibits robustness in real-world task execution. We highly recommend readers to view our \textbf{supplementary video} for a richer visualization of UniAct's performance across diverse scenarios.

\section{Implementation details}\label{sec:implementation}

\subsection{Tokenization}

\paragraph{Network design} The model employs a convolutional autoencoder architecture with finite scalar quantization (FSQ) for discrete latent representation learning. The encoder-decoder framework processes sequences of shape (B, N, D) where B is batch size, N is sequence length, and D is feature dimension.

The encoder consists of an input projection layer followed by two conv blocks with increasing channel capacity. Each conv block contains a strided 1D convolution with kernel size 7 and a residual block. The residual blocks combine 1D convolutions with GroupNorm and per-position MLPs that apply LayerNorm and GELU activations. The encoder reduces the sequence length by a factor of 2 (from N to N/2) while projecting to a 5-dimensional latent space.

The decoder mirrors the encoder architecture with transposed 1D convolutions for upsampling. It takes the quantized latents and upsamples them through upsampling blocks, doubling the temporal resolution while reducing channel dimensions. The final projection layer reconstructs the original input dimension. The model uses hidden dimensions of 256 channels in intermediate layers, with expansion factors in the residual blocks for increased representational capacity. All convolution operations use appropriate padding to maintain temporal alignment throughout the network.

In ablation studies described in~\cref{sec:exp}, we evaluated two architectural modifications to understand the importance of codebook capacity and temporal resolution. As shown in~\cref{tab:multimodal_control,tab:motion_tracking}, reducing the codebook size to 0.25× by decreasing quantization levels resulted in performance degradation, indicating that sufficient discrete representation capacity is crucial for capturing the data distribution. Similarly, increasing the downsampling rate to 4 also decreased performance, demonstrating that maintaining adequate temporal resolution in the latent space is essential for accurate reconstruction. Excessive temporal resolution increases computational latency during motion generation. To balance motion quality with real-time performance, we adopt a downsampling rate of 2.

\paragraph{Codebook usage}
FSQ adapts its codebook size to match the complexity of different modalities. For robot motion, the FSQ quantizer discretizes the continuous degrees of freedom using predefined quantization levels [8, 8, 8, 6, 5] across 5 latent dimensions, yielding a codebook of 8×8×8×6×5=15,360 discrete codes. This larger codebook captures the nuanced variations in joint configurations and dynamic movements required for expressive robot control. In contrast, music representations utilize 6,144 codes to encode audio features, while trajectory data requires only 60 codes due to its lower-dimensional complexity and smoother spatial characteristics.

Our approach directly learns robot motion in the robot's native kinematic space, eliminating the need for post-processing retargeting steps. This end-to-end learning strategy contrasts with conventional pipelines that first generate human motion using human models (such as SMPL-X), then apply optimization-based retargeting to map the motion onto humanoid robots' workspace. Such two-stage approaches introduce cumulative errors from body proportion mismatches, joint limit violations, and the fundamental differences between human and robot morphology. Our quantitative results demonstrate that direct robot motion embedding achieves superior tracking accuracy and naturalness compared to retargeting-based methods, while also reducing computational overhead by avoiding the intermediate human representation and complex optimization procedures required for motion transfer.

The unified codebook is partitioned to accommodate multiple modalities while preserving the original text vocabulary. As listed in~\cref{tab:codebook_allocation}, we allocate non-overlapping index ranges for each modality: indices 0–130,076 are reserved for the original text tokens, ensuring compatibility with pretrained language models. Indices 130,077–130,078 correspond to the special tokens \texttt{<SOM>} (start of motion) and \texttt{<EOM>} (end of motion). Subsequently, indices 130,079–145,438 are designated for robot motion codes, 145,439–151,582 represent music tokens, and indices 151,583–151,642 encode trajectory representations. This design enables seamless multi-modal generation within a single autoregressive framework.

\begin{table}[h]
\scriptsize
\centering
\caption{Codebook allocation across modalities.}
\begin{tabular}{lcc}
\hline
Modality & Index Range & Codebook Size \\
\hline
Text & 0 -- 130,076 & 130,077 \\
\texttt{<SOM>} and \texttt{<EOM>} & 130,077 -- 130,078 & 2 \\
Robot Motion & 130,079 -- 145,438 & 15,360 \\
Music & 145,439 -- 151,582 & 6,144 \\
Trajectory & 151,583 -- 151,642 & 60 \\
\hline
\end{tabular}
\label{tab:codebook_allocation}
\end{table}

\subsection{Motion tracking}

We implement our motion tracking pipeline using PPO to train policies on the Unitree G1 humanoid robot. The framework processes hours-long reference motions from the UA-Net dataset using a unified set of hyperparameters across all motions.

We adapt the motion tracking policy from BeyondMimic by removing global orientation from the reference motion observation, allowing the policy to focus on relative joint configurations:
\begin{equation}
\mathbf{o}_t = [\mathbf{q}_t^\text{ref}, \dot{\mathbf{q}}_t^\text{ref}, \mathbf{q}_t^\text{curr}, \dot{\mathbf{q}}_t^\text{curr}, \mathbf{g}_t, \mathbf{\omega}_t, \mathbf{a}_{t-1}]
\end{equation}
where $\mathbf{q}_t^\text{ref}$ and $\dot{\mathbf{q}}_t^\text{ref}$ are the decoded reference position and velocity, $\mathbf{q}_t^\text{curr}$ and $\dot{\mathbf{q}}_t^\text{curr}$ are the current robot joint states, $\mathbf{g}_t$ represents the gravity vector in the robot frame, $\mathbf{\omega}_t$ represents the angular velocity, and $\mathbf{a}_{t-1}$ represents the robot action at previous timestep. We use asymmetric actor-critic training where the critic additionally receives per-body relative poses for direct Cartesian error estimation.

The tracker outputs joint target positions $\mathbf{p}_t$ that drive the robot to follow the generated motion while maintaining balance and physical feasibility. These are converted to torques through PD control:
\begin{equation}
\boldsymbol{\tau}_j = k_{p,j}(\mathbf{p}_{t,j} - \mathbf{q}_{t,j}^\text{curr}) - k_{d,j}\dot{\mathbf{q}}_{t,j}^\text{curr}
\end{equation}
where $\boldsymbol{\tau}_j$ is the derived torque applied to each robot joint.

Joint stiffness and damping follow:
\begin{equation}
k_{p,j} = I_j \omega_n^2, \quad k_{d,j} = 2 I_j \zeta \omega_n
\end{equation}
with natural frequency $\omega_n = 10$ Hz, overdamped ratio $\zeta = 2$, and reflected inertia $I_j = k_{g,j}^2 I_{\text{motor},j}$.

\paragraph{Reward design}

The reward function primarily consists of tracking rewards that measure motion accuracy and penalty terms for physical constraints. The tracking rewards include matching the root orientation, body link positions and orientations relative to the root frame, and linear/angular velocities of all tracked links to ensure accurate motion reproduction. Key penalties include action rate regularization to reduce jitter, joint limit violations to prevent hardware damage, and undesired contacts to avoid collisions between non-end-effector body parts and the environment. For more details, please refer to~\cref{tab:beyondmimic}.

\paragraph{Domain randomization}

We randomize ground friction $\mu \sim \mathcal{U}(0.5, 1.5)$, joint offsets $\Delta q_j \sim \mathcal{U}(-0.05, 0.05)$ rad, and center of mass position $\Delta \mathbf{p}_{\text{CoM}} \sim \mathcal{U}(-0.02, 0.02)$ m.

\paragraph{Training configuration}

Networks use MLPs with [2048, 1024, 512, 256, 128] hidden units and ELU activations. PPO training uses clip range 0.2, learning rate $1 \times 10^{-3}$, discount $\gamma = 0.99$, GAE $\lambda = 0.95$, with 16,384 environments and control frequency 200 Hz (decimation=4).

\paragraph{Deployment}

Policies are exported as PyTorch (.pt) files and deployed at 50 Hz. Each inference step takes about 7ms on an RTX 4090 GPU.

\begin{table}[h]
\caption{Reward components and weights for OmniH2O~\cite{he2024omnih2o}.}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccc}
\hline
\textbf{Term} & \textbf{Expression} & \textbf{Weight} \\
\hline
\multicolumn{3}{c}{\textbf{Penalty}} \\
\hline
DoF position limits & $\mathds{1}(d_t \notin [q_{\min}, q_{\max}])$ & -1500 \\
Termination & $\mathds{1}_{\text{termination}}$ & -250 \\
\hline
\multicolumn{3}{c}{\textbf{Regularization}} \\
\hline
Lower-body action rate & $\|a_t^{\text{lower}} - a_{t-1}^{\text{lower}}\|_2^2$ & -2 \\
Upper-body action rate & $\|a_t^{\text{upper}} - a_{t-1}^{\text{upper}}\|_2^2$ & -4 \\
Torque & $\|\tau_t\|$ & -0.0005 \\
Slippage & $\|v_t^{\text{feet}}\|_2^2 \times \mathds{1}(F_{\text{feet}} \geq 1)$ & -5 \\
\hline
\multicolumn{3}{c}{\textbf{Task Reward}} \\
\hline
DoF position & $\exp(-0.25\|d_t - \tilde{d}_t\|_2)$ & 100 \\
DoF velocity & $\exp(-0.25\|\dot{d}_t - \dot{\tilde{d}}_t\|_2^2)$ & 20 \\
Body position & $\exp(-0.5\|p_t - \tilde{p}_t\|_2^2)$ & 50 \\
Body rotation & $\exp(-0.1\|\theta_t \ominus \tilde{\theta}_t\|)$ & 50 \\
Body velocity & $\exp(-10.0\|v_t - \tilde{v}_t\|_2)$ & 20 \\
Body angular velocity & $\exp(-0.01\|\omega_t - \tilde{\omega}_t\|_2)$ & 20 \\
\hline
\end{tabular}
}
\label{tab:omnih2o}
\end{table}



\begin{table}[h]
\caption{Reward components and weights for BeyondMimic~\cite{liao2025beyondmimic}.}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccc}
\hline
\textbf{Term} & \textbf{Expression} & \textbf{Weight} \\
\hline
\multicolumn{3}{c}{\textbf{Penalty}} \\
\hline
Action rate & $\|\bs{a}_t-\bs{a}_{t-1}\|_2^2$ & -0.1 \\
Joint limit & $\sum_{j} \mathds{1}[\bs{q}_{t,j} \notin [\bs{q}_{t,j}^{\text{min}}, \bs{q}_{t,j}^{\text{max}}]]$ & -10.0 \\
Undesired contacts & $\sum_{c \notin \{\text{ankles, wrists}\}} \mathds{1}[\|\bs{F}_c\|>1.0\text{N}]$ & -0.1 \\
\hline
\multicolumn{3}{c}{\textbf{Task Reward}} \\
\hline
Root orientation & $\exp\!\big(- \|\bs{o}^p_{t,r}-\bs{o}^g_{t,r}\|_2^2 / 0.4^2\big)$ & 0.5 \\
Body link pos (rel.) & $\exp\!\Big(-\tfrac{1}{|\mathcal{B}|}\!\sum_{b\in\mathcal{B}}\|\bs{p}^{p,\text{rel}}_{t,b}-\bs{p}^{g,\text{rel}}_{t,b}\|_2^2 / 0.3^2\Big)$ & 1.0 \\
Body link ori (rel.) & $\exp\!\Big(-\tfrac{1}{|\mathcal{B}|}\!\sum_{b\in\mathcal{B}} \|\bs{o}^{p,\text{rel}}_{t,b}-\bs{o}^{g,\text{rel}}_{t,b}\|_2^2 / 0.4^2\Big)$ & 1.0 \\
Body link lin. vel & $\exp\!\Big(-\tfrac{1}{|\mathcal{B}|}\!\sum_{b\in\mathcal{B}}\|\bs{v}^p_{t,b}-\bs{v}^g_{t,b}\|_2^2 / 1.0^2\Big)$ & 1.0 \\
Body link ang. vel & $\exp\!\Big(-\tfrac{1}{|\mathcal{B}|}\!\sum_{b\in\mathcal{B}}\|\bs{\omega}^p_{t,b}-\bs{\omega}^g_{t,b}\|_2^2 / 3.14^2\Big)$ & 1.0 \\
\hline
\end{tabular}
}
\label{tab:beyondmimic}
\end{table}





\section{Baseline methods}
We apply OmniH2O, UH-1, and LangWBC as our baselines. For OmniH2O, we adapt the original settings from the H1 robot to G1, with the parameters shown in~\cref{tab:omnih2o}. We leverage Qwen2.5-3B throughout these comparisons.

For UH-1, we adopt the end-to-end configuration where the method directly generates robotic actions $A_{robot}$ from text input for open-loop control (text-to-action). To ensure fair comparison with our approach, we train the control policy using the same architecture and training procedure as the motion tracker in UniAct. Specifically, the policy network learns to map text embeddings directly to joint-level control commands without intermediate motion representation. The parameters are adapted from the original Unitree H1-2 configuration to accommodate the G1 robot.

For LangWBC, we reimplement the method using the BeyondMimic tracker as the teacher policy with reward formulation in~\cref{tab:beyondmimic}. We maintain the original CVAE architecture and DAgger training but scale to 4,096 parallel environments. Unlike the original implementation that tracks only root displacement, we extend the loss computation to whole-body tracking across all keypoints, enabling more accurate motion reproduction on the G1 robot.

We employ the motion diffusion model (MDM) as the motion generator for two-stage baseline methods. The MDM model was trained using motions from the UA-Net training set, which were converted to SMPL-X format for compatibility.


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.48\linewidth]{figures/mpjpe_comparison.pdf}
    \hfill
    \includegraphics[width=0.48\linewidth]{figures/success_rate_comparison.pdf}
    \caption{\textbf{Performance comparison between BeyondMimic and BeyondMimic + FSQ (ours) under different noise scales.} (left) MPJPE comparison. (right) Success rate comparison. As the noise scale progressively increases, BeyondMimic exhibits significant performance degradation, whereas BeyondMimic + FSQ (ours) maintains relatively low MPJPE and high success rates even at the maximum noise scale (×8), which demonstrates that our quantization approach effectively constrains motions to feasible spaces, enhancing robustness.}
    \label{fig:fsq_tracking_performance_comparison}
\end{figure*}

\section{UA-Net dataset}

\subsection{Trajectory expansion with motion-matching}
We collected approximately 20 minutes of human walking motion data on flat terrain using the OptiTrack MoCap system. To obtain paired data of arbitrary trajectories and walking motions, we augmented this dataset using motion matching, expanding the walking motion data from 20 minutes in the UA-Net dataset to over 10 hours. This motion-matching-based augmentation pipeline preserves natural locomotion characteristics while following diverse, non-repetitive trajectories. The motion matching pipeline is present in~\cref{fig:motionmatching}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/motion_matching.pdf}
    \caption{\textbf{Overview of motion-matching-based walking motion expansion}. To expand the human walking trajectories in the UA-Net dataset from 20 minutes to over 10 hours, we employ a motion-matching-based augmentation approach. The original motion sequences are segmented into short clips, with each frame represented by features capturing pose, velocity, and future trajectory information. During synthesis, the system continuously searches for optimal clip transitions based on feature similarity and blends them smoothly.}
    \label{fig:motionmatching}
\end{figure}

\paragraph{Feature extraction}
In motion matching, each frame is represented by a comprehensive feature vector containing root position and orientation, relative joint positions for lower-body joints (foot and ankles), root and foot velocities, future trajectory points sampled at 20, 40, and 60 frames ahead, and gait phase information derived from foot contact patterns. These features capture both the instantaneous pose and the movement intention, enabling accurate matching between motion clips.

\paragraph{Segmentation process}
The original 20-minute sequences are segmented into overlapping clips of 2-4 seconds, with cut points determined by gait cycle boundaries at heel-strike events and steady-state walking phases where acceleration is minimal. Each segment maintains at least two complete gait cycles and is annotated with metadata, including walking speed and turning angle. The overlapping strategy ensures multiple transition possibilities from each clip.

\paragraph{Matching and synthesis}
During synthesis, the system searches for optimal transitions when approaching the last 10 frames of the current clip. The matching cost function evaluates feature similarity through weighted Euclidean distance, velocity consistency, trajectory alignment, and foot contact states. To ensure diversity, we implement a history buffer that penalizes recently used clips and probabilistically select from the top-5 candidates rather than always choosing the best match.

Transitions are blended over 10 frames using spherical linear interpolation for rotations and cubic interpolation for positions. Post-processing applies inverse kinematics to maintain foot contacts during stance phases and smooths trajectories to eliminate artifacts. The pipeline continuously monitors quality metrics, including foot sliding and acceleration discontinuities, automatically filtering problematic sequences.

This approach successfully synthesizes over 10 hours of varied, natural walking motions from the original 20-minute MoCap data, providing sufficient diversity for training trajectory following.

\subsection{Text-to-motion from MoCap}

The UA-Net dataset comprises over 10,000 expressive motion sequences with meticulously curated motion descriptions. We systematically cover 1,400 common action verbs, representing 1.8× the vocabulary coverage of HumanML3D dataset. For each verb, we compose contextually appropriate sentences that naturally incorporate the verb as the primary action descriptor. High-frequency verbs receive additional instances to reflect their prevalence in real-world applications, with frequently used actions like `walk,' `run,' and `turn' appearing in multiple distinct motion descriptions to ensure comprehensive coverage of common movements.

We employed 10 professional MoCap actors (4 male, 6 female), carefully selected for similar body proportions to minimize morphological variation in the dataset. All actors possess foundational dance training, ensuring they can execute movements with proper body control and spatial awareness. During capture sessions, actors were instructed to perform motions with slight expressiveness beyond everyday movements, adding subtle stylistic flourishes and dynamic variations that enhance the dataset's richness while maintaining naturalness. This directive encouraged actors to interpret each motion with personality rather than mechanical execution, resulting in more engaging and diverse performances that better reflect how humans naturally move when given verbal instructions.




\section{Robustness analysis under input corruption}

To evaluate whether our discrete representation can effectively refine noisy inputs, we introduce Gaussian noise and temporal jitter to UA-Net motions to simulate low-quality input data. The noise model mimics low-quality MoCap data by incorporating three primary components that represent common tracking artifacts. Given an input motion sequence $\mathbf{X} \in \mathbb{R}^{N \times D}$ with $N$ frames and $D = 29$ degrees of freedom, we generate the noisy output as:
\begin{equation}
\tilde{\mathbf{X}} = \mathbf{X} + \mathbf{n}_{\text{base}} + \mathbf{n}_{\text{burst}} + \mathbf{n}_{\text{jitter}}
\end{equation}
where $\mathbf{n}_{\text{base}} \sim \mathcal{N}(0, \sigma_{\text{base}}^2\mathbf{I})$ with $\sigma_{\text{base}} = 0.01$ represents baseline sensor noise inherent in all motion capture systems. The burst noise $\mathbf{n}_{\text{burst}}$ simulates temporary tracking failures that occur with probability $p_{\text{burst}} = 0.05$ per frame, affecting random subsets of dimensions with temporally correlated Gaussian perturbations $\mathcal{N}(0, \sigma_{\text{burst}}^2\mathbf{I})$ where $\sigma_{\text{burst}} = 0.1$ over durations of 8-20 frames. The jitter noise $\mathbf{n}_{\text{jitter}}$ models sudden tracking spikes that occur with probability $p_{\text{jitter}} = 0.001$ per dimension per frame, introducing large-magnitude disturbances drawn from $\mathcal{N}(0, \sigma_{\text{jitter}}^2\mathbf{I})$ where $\sigma_{\text{jitter}} = 0.3$. After processing these corrupted motions through our discrete representation, we compare the tracking performance against the original unperturbed references to assess the quantization's denoising capabilities. 

As shown in \cref{tab:motion_tracking}, all quantization settings achieve significantly better tracking performance compared to the baseline tracking method, where corrupted motions are directly fed into the BeyondMimic motion tracker. This demonstrates that the discrete token representation effectively filters out noise by constraining motions to a finite, well-explored space of learned motion patterns. The quantization process inherently rejects out-of-distribution perturbations and projects noisy inputs onto the manifold of plausible human motions, thereby significantly enhancing tracking robustness even under substantial input corruption.

To further validate the advantages of token-based motion representation, we evaluated the performance of both BeyondMimic and BeyondMimic + FSQ (ours) under varying noise scales. As shown in~\cref{fig:fsq_tracking_performance_comparison}, as the noise scale progressively increases, BeyondMimic exhibits significant performance degradation, whereas BeyondMimic + FSQ (ours) maintains relatively low MPJPE and high success rates even at the maximum noise scale (×8). This demonstrates that our method can effectively restore the quality of out-of-distribution low-quality data to a certain extent, thereby providing more feasible reference motions for the motion tracking policy.


\section{Compositional cross-modal control}

UniAct extends naturally to cross-modal humanoid control tasks, where robots must simultaneously process and execute instructions from multiple input modalities. This capability is exemplified by scenarios requiring the robot to perform expressive gestures, such as waving, while simultaneously following a specified trajectory. Such multi-modal control is crucial for practical deployment scenarios where robots must navigate through environments while maintaining meaningful interactions with humans.

Our approach leverages a key observation: expressive semantic actions predominantly manifest in the upper body of humanoid robots, while trajectory following primarily engages lower-body locomotion. This natural decomposition enables a compositional generation strategy where we independently generate motions from language and trajectory instructions, then synthesize them by combining the upper-body motion from text-conditioned generation with the lower-body motion from trajectory-conditioned generation. We establish the pelvis as the anatomical boundary, with the pelvis itself belonging to the lower body to maintain stable locomotion dynamics. The composed motion is subsequently forwarded to the motion tracking policy for real-world execution.

To ensure robust tracking of these compositionally generated motions, we implement a fine-tuning strategy for the tracking policy. During fine-tuning, we systematically compose motions by randomly pairing lower-body segments from trajectory data with upper-body segments from other motion categories within the UA-Net dataset. This augmentation strategy exposes the tracking policy to motion patterns structurally similar to those encountered during cross-modal inference, enabling successful execution of previously unseen cross-modal compositions. \cref{fig:cross_modal2motion_qual} illustrates the results from our cross-modal experiments, demonstrating coherent execution of combined instructions.

This compositional approach enables zero-shot generalization to novel motion-trajectory combinations. For instance, despite the training dataset containing only stationary versions of actions such as `making a phone call' or `playing drums', our method successfully controls the robot to perform these actions while following arbitrary trajectories. This capability significantly expands the robot's behavioral diversity without requiring exhaustive data collection for every possible combination of actions and trajectories, thereby demonstrating the scalability and practical utility of our framework for real-world humanoid deployment.




\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/text2motion_qualitative_results.png}
    \caption{\textbf{Qualitative results of language-conditioned humanoid control}.}
    \label{fig:text2motion_qual}
\end{figure*}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/music2motion_qualitative_results.png}
    \caption{\textbf{Qualitative results of music-conditioned humanoid control}.}
    \label{fig:music2motion_qual}
\end{figure*}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/trajectory2motion_qualitative_results.png}
    \caption{\textbf{Qualitative results of trajectory-conditioned humanoid control}.}
    \label{fig:traj2motion_qual}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/gvhmr2motion_qualitative_results.png}
    \caption{\textbf{Qualitative results of human-to-humanoid motion control}.}
    \label{fig:gvmhr2motion_qual}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/cross_modal2motion_qualitative_results.png}
    \caption{\textbf{Qualitative results of cross-modal humanoid control}.}
    \label{fig:cross_modal2motion_qual}
\end{figure*}




% \pagebreak
% \clearpage
% \clearpage
% {
%     \small
%     \bibliographystyle{ieeenat_fullname}
%     \bibliography{reference_header,ref_supp}
% }
